Andes: Defining and Enhancing Quality-of-Experience in LLM-Based Text Streaming Services

Large language models (LLMs) are now at the core of conversational AI services such as real-time translation and chatbots, which provide live user interaction by incrementally streaming text to the user. However, existing LLM serving systems fail to provide good user experience because their optimization metrics are not always aligned with user experience. In this paper, we first introduce and define the notion of Quality-of-Experience (QoE) for text streaming services by considering each user's end-to-end interaction timeline. Based on this, we propose Andes, a QoE-aware LLM serving system that enhances user experience by ensuring that users receive the first token promptly and subsequent tokens at a smooth, digestible pace, even during surge periods. This is enabled by Andes's preemptive request scheduler that dynamically prioritizes requests at the token granularity based on each request's expected QoE gain and GPU resource usage. Our evaluations demonstrate that, compared to state-of-the-art LLM serving systems, Andes improves the average QoE by up to $4.7\times$ given the same GPU resource, or saves up to 61% GPU resources while maintaining the same high QoE.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=andes-osdi25


PDF = andes-osdi25.pdf 

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %, %,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done



%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	#pdflatex samples.ins 
	for texfile in *.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


# samples/$(PACKAGE).cls: $(PACKAGE).cls
ACM-Reference-Format.bst: ACM-Reference-Format.bst

abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > abbrev.bib 


%.bbx: %.bbx
%.cbx: %.cbx
%.dbx: %.dbx
%.lbx: %.lbx

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	  ACM-Reference-Format.bst \
	*.log *.aux *.out \
	*.bbl *.blg *.cut \
	acm-jdslogo.png \
	*.run.xml *.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)    \ 

distclean: clean
	$(RM)  *.pdf andes-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	*.cls ACM-Reference-Format.*

split:
	qpdf ${PDF} --pages . 1-14 -- ${PACKAGE}-main.pdf
	qpdf ${PDF} --pages . 15-z -- ${PACKAGE}-apdx.pdf



.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> pages/client.tex <==
\section{Client Token Buffering}
 \label{sec:token-buffer} 

 
In this section, we discuss the client-side token buffer, which is designed to ensure a smooth and uninterrupted flow of tokens to the user. 
The buffer's primary function is to store excess tokens generated by the server, enabling a consistent delivery rate that aligns with the user's expected Time to First Token (TTFT) and Token Delivery Speed (TDS).
 Additionally, it decouples user experience from server behavior, as it helps abstract away variations in server-side performance, allowing for uninterrupted token delivery even when the server temporarily pauses the request.
Finally, in the face of network delays, the buffer ensures that users continue to receive tokens, masking any temporary communication issues.

\begin{figure}[t!]
  \centering
  \includegraphics[trim=90 100 120 50,clip,width=\linewidth]{client-buffer.pdf} 
    \caption{Client buffer example to show it smooths the token delivery from server generation pause and fluctuation, and aligns with expected speed.}
    \label{fig:client-buffer}
\end{figure}

As illustrates in Figure~\ref{fig:client-buffer}, the token buffer introduces several optimizations to further enhance the user experience:
\begin{enumerate} 
\item 
Chunk Fetching: Instead of fetching tokens one by one, which can lead to network underutilization and latency, the buffer can fetch of larger token chunks after a brief interval when the buffer is filled.

\item 
End-of-Response Flushing: Upon detecting the end of a response, the buffer can promptly flush all remaining tokens to the user. This eliminates the need for further buffering and allows for the immediate display of the complete response.

\item 
Server Load Awareness: If the system can detect low server contention, it may temporarily disable the client buffer, allowing tokens to be displayed more rapidly. 
This can be particularly useful when the server can deliver the entire response quickly, as it aligns with user expectations for immediate information.

\end{enumerate} 



Client-side token buffer complements our server-side QoE-aware scheduling, ensuring that the strategic request scheduling on the server are reflected in smooth and consistent token delivery to the user. 
Together, these mechanisms optimize QoE by aligning token delivery with user expectations, both at the server level and during the final delivery stage.




% 
%**Implementation Details:**
%The implementation of client-side buffering involves the following key aspects:
%
%1. **Buffer Size Management:** Determining the optimal size of the buffer to balance between memory usage and the need for seamless token delivery.
%2. **Token Fetching Strategy:** Developing algorithms to decide when and how many tokens to fetch from the server, based on the buffer's state and network conditions.
%3. **End-of-Sentence Detection:** Implementing mechanisms to detect the completion of sentences or token sequences, enabling timely flushing of the buffer.
%4. **Adaptation to Network Conditions:** Dynamically adjusting the token fetching strategy based on real-time network performance metrics.
%
%By incorporating these implementation details, the client-side token buffer effectively enhances the user experience in LLM text streaming services, ensuring a smooth and enjoyable interaction with the system.
